Robust Multi-Agent Reinforcement Learning with Social Empowerment for Coordination and Communication

We consider the problem of robust multi-agent reinforcement learning (MARL) for cooperative communication and coordination tasks. MARL agents, mainly those trained in a centralized way, can be brittle because they can adopt policies that act under the expectation that other agents will act a certain way rather than react to their actions. Our objective is to bias the learning process towards finding strategies that remain reactive towards others' behavior. Social empowerment measures the potential influence between agents' actions. We propose it as an additional reward term, so agents better adapt to other agents' actions. We show that the proposed method results in obtaining higher rewards faster and a higher success rate in three cooperative communication and coordination tasks.

==> tmp.tex <==

This paper clearly states what claims are being investigated.

Yes
Partial
No
• Reproducibility checklist (2) *
This paper explains how the results substantiate the claims.

Yes
Partial
No
• Reproducibility checklist (3) *
This paper explicitly identifies limitations or technical assumptions.

Yes
Partial
No
• Reproducibility checklist (4) *
This paper includes a conceptual outline and/or pseudocode description of AI methods introduced.

Yes
Partial
No
Not applicable
• Reproducibility checklist (5) *
Does this paper make theoretical contributions?

Yes
No
• Reproducibility checklist (5.1) *
All assumptions and restrictions are stated clearly and formally.

Yes
Partial
No
• Reproducibility checklist (5.2) *
\textbf{All novel claims are stated formally (e.g., in theorem statements).}

Yes
Partial
No
• Reproducibility checklist (5.3) *
Proofs of all novel claims are included.

Yes
Partial
No
• Reproducibility checklist (5.4) *
Proof sketches or intuitions are given for complex and/or novel results.

Yes
Partial
No
• Reproducibility checklist (5.5) *
Appropriate citations to theoretical tools used are given.

Yes
Partial
No
• Reproducibility checklist (6) *
Does this paper rely on one or more data sets?

Yes
No
• Reproducibility checklist (7) *
Does this paper include computational experiments?

Yes
No
• Reproducibility checklist (7.1) *
All source code required for conducting experiments is included in a code appendix.

Yes
Partial
No
• Reproducibility checklist (7.2) *
\textbf{All source code required for conducting experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes.}

Yes
Partial
No
• Reproducibility checklist (7.3) *
\textbf{If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results.}

Yes
Partial
No
Not applicable
• Reproducibility checklist (7.4) *
This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks.

Yes
Partial
No
• Reproducibility checklist (7.5) *
This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics.

Yes
Partial
No
• Reproducibility checklist (7.6) *
This paper states the number of algorithm runs used to compute each reported result.

Yes
No
• Reproducibility checklist (7.7) *
Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information.

Yes
\textbf{No}
• Reproducibility checklist (7.8) *
This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments.

Yes
Partial
No
\textbf{Not applicable}
• Reproducibility checklist (7.9) *
This paper states the number and range of values tried per (hyper-)parameter during development of the paper, along with the criterion used for selecting the final parameter setting.

Yes
Partial
No
Not applicable
Submit Cancel
© 2020 Microsoft Corporation About CMT | Help | Terms of Use | Privacy & Cookies | Request CMT SiteTwitter CMT Support
